SC-LiDAR-SLAM: a Front-end Agnostic Versatile LiDAR SLAM System

Accurate 3D point cloud map generation is a core task for various robot missions or even for data-driven urban analysis. To do so, light detection and ranging (LiDAR) sensor-based simultaneous localization and mapping (SLAM) technology have been elaborated. To compose a full SLAM system, many odometry and place recognition methods have independently been proposed in academia. However, they have hardly been integrated or too tightly combined so that exchanging (upgrading) either single odometry or place recognition module is very effort demanding. Recently, the performance of each module has been improved a lot, so it is necessary to build a SLAM system that can effectively integrate them and easily replace them with the latest one. In this paper, we release such a front-end agnostic LiDAR SLAM system, named SC-LiDAR-SLAM. We built a complete SLAM system by designing it modular, and successfully integrating it with Scan Context++ and diverse existing opensource LiDAR odometry methods to generate an accurate point cloud map

==> src/ack.tex <==
\section*{Acknowledgment}

Thank you. supported by ...

==> src/fig/fig_livox.tex <==
%FIGURE key effect
\begin{figure}[!t]
  \centering
  \includegraphics[width=0.89\columnwidth, trim = 0 0 0 0, clip]{fig/scfastlio}
  \caption{
    todo 
  }
  \label{fig:livox}
  % \vspace{-3mm}
\end{figure}
%FIGURE key effect 

